MACE: Mass Concept Erasure in Diffusion Models

The rapid expansion of large-scale text-to-image diffusion models has raised growing concerns regarding their potential misuse in creating harmful or misleading content. In this paper, we introduce MACE, a finetuning framework for the task of mass concept erasure. This task aims to prevent models from generating images that embody unwanted concepts when prompted. Existing concept erasure methods are typically restricted to handling fewer than five concepts simultaneously and struggle to find a balance between erasing concept synonyms (generality) and maintaining unrelated concepts (specificity). In contrast, MACE differs by successfully scaling the erasure scope up to 100 concepts and by achieving an effective balance between generality and specificity. This is achieved by leveraging closed-form cross-attention refinement along with LoRA finetuning, collectively eliminating the information of undesirable concepts. Furthermore, MACE integrates multiple LoRAs without mutual interference. We conduct extensive evaluations of MACE against prior methods across four different tasks: object erasure, celebrity erasure, explicit content erasure, and artistic style erasure. Our results reveal that MACE surpasses prior methods in all evaluated tasks. Code is available at https://github.com/Shilin-LU/MACE.

==> sec/preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
\begin{align} 
	\mathcal{L}_\text{LDM} = \mathbb{E}_{\bfz \sim \mathcal{E}(\bfx),\bfy,\boldsymbol{\epsilon} \sim \mathcal{N}(0,1), t} \left[ \left\| \boldsymbol{\epsilon}  - \boldsymbol{\epsilon}_{\boldsymbol{\theta}}(\bfz_t, t, \boldsymbol{\tau}) \right\|^2_2 \right],
	\label{eq:ldm}
\end{align}

==> sec/problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem}

%We seek a forgetting mechanism, denoted by a function \( f(\cdot, \cdot) \). This function takes two inputs: a pretrained generative model \( \mathcal{G} \) and a set of concepts \( C_f = \{c_1, c_2, \ldots, c_m\} \) meant for forgetting. It returns a refined model, \( \mathcal{G}' = f(\mathcal{G}, C_f) \), which no longer generates concepts in $C_f$. Notably, a concept $c$ can be conveyed using various phrases. We refer to the target phrase as $p_0$, which is the input for erasing, and its synonyms as $\{ p_1,p_2,\ldots,p_n\}$. Based on practical needs, we outline the following desiderata for a method \( f(\cdot, \cdot) \) aimed at addressing this challenge:
%
%\begin{itemize}[itemsep=0.1em, topsep=0.1em]
%	\item \textbf{Efficacy:} When conditioned on the target phrase $p_0$ (e.g., `construction crane’) within a specific context, the outputs from the refined model should have limited semantic alignment with the expressed concept $c_0$ (i.e., a construction apparatus) in comparison to the original model. Yet, these outputs should remain within the natural image manifold, either aligning with a generic background category (e.g., sky or street), or defaulting to the super-category of the concept \( c_0 \), if one exists.
%	
%	\item \textbf{Generality:} If the refined model is conditioned on prompts that involve either a synonym of $p_0$ (e.g., derrick) or $p_0$ placed in varied contexts (e.g., at the beach), its behavior should mirror that when conditioned on \( p_0 \).
%	
%	\item \textbf{Specificity:} If the refined model is conditioned on prompts with phrases that are semantically irrelevant to the concept $c_0$ (e.g., car) or the same phrase signifying a different concept (e.g., crane denoting an avian species), its output distribution should closely align with that of the original model.
%\end{itemize}

We aim to develop a framework to erase a large volume of concepts from the pretrained T2I diffusion model. This framework takes as input a pretrained model and a set of target phrases expressing concepts to be removed. It returns a finetuned model that is incapable of generating images depicting the concepts targeted for erasing. An effective erasure framework should fulfill the following criteria:

\begin{itemize}[itemsep=0.1em, topsep=0.1em]
	\item \textbf{Efficacy (block target phrases):} If the finetuned model is conditioned on prompts with those target phrases, its outputs should have limited semantic alignment with the prompts. Yet, the outputs should still appear natural, either aligning with a generic category (e.g., sky), or defaulting to the super-category of the concept, if one exists.
	
	\item \textbf{Generality (block synonyms):} The model should also prevent the generation of images semantically related to any synonyms of the targeted phrases, ensuring that the erasure is not limited to the exact wording of the prompts.
	
	\item \textbf{Specificity (preserve unrelated concepts):} If the finetuned model is conditioned on prompts that are semantically unrelated to the erased concepts, its output distribution should closely align with that of the original model.
\end{itemize}

